LiV-GS: LiDAR-Vision Integration for 3D Gaussian Splatting SLAM in Outdoor Environments

We present LiV-GS, a LiDAR-visual SLAM system in outdoor environments that leverages 3D Gaussian as a differentiable spatial representation. Notably, LiV-GS is the first method that directly aligns discrete and sparse LiDAR data with continuous differentiable Gaussian maps in large-scale outdoor scenes, overcoming the limitation of fixed resolution in traditional LiDAR mapping. The system aligns point clouds with Gaussian maps using shared covariance attributes for front-end tracking and integrates the normal orientation into the loss function to refines the Gaussian map. To reliably and stably update Gaussians outside the LiDAR field of view, we introduce a novel conditional Gaussian constraint that aligns these Gaussians closely with the nearest reliable ones. The targeted adjustment enables LiV-GS to achieve fast and accurate mapping with novel view synthesis at a rate of 7.98 FPS. Extensive comparative experiments demonstrate LiV-GS's superior performance in SLAM, image rendering and mapping. The successful cross-modal radar-LiDAR localization highlights the potential of LiV-GS for applications in cross-modal semantic positioning and object segmentation with Gaussian maps.

==> table/close-loop.tex <==
\begin{table}[h]
\centering
\begin{minipage}{0.48\textwidth}
\centering
\caption{Quantitative Analysis for Tracking Accuracy}
\label{table:tracking_accuracy}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{\textbf{HKU Park}} \\
\cmidrule(lr){2-4}
\textbf{Methods}  & $t_{rel}\downarrow$ & $r_{rel}\downarrow$ & $t_{abs}\downarrow$ \\
\midrule
NeRF-LOAM                   & 0.718 & 21.95  & 0.617 \\
HDL-graph-SLAM              & 0.552 & 17.336 & 0.772 \\
ORB-SLAM3                   & 0.566 & 19.226 & 0.698 \\
SplaTAM                     & 0.629 & 18.772 & 0.585 \\
MonoGS                      & 0.535 & 17.501 & 0.691 \\
Gaussian-SLAM               & 0.655 & 20.962 & 0.444 \\
GS-ICP-SLAM                 & 0.733 & 22.118 & 0.364 \\
Ours                        & 0.586 & 0.546 & 0.775 \\
\bottomrule
\end{tabular}
}
\end{minipage}%
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{Quantitative Analysis for Rendering}
\label{table:rendering}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{\textbf{HKU Park}} \\
\cmidrule(lr){2-4}
\textbf{Methods} & \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
\midrule
3DGS                      & 0.868 & 25.776 & 0.247 \\
GS-ICP-SLAM               & 0.446 & 11.949 & 0.813 \\
NeRF++                    & 0.581 & 12.256 & 0.791 \\
SplaTAM                   & 0.235 & 10.501 & 0.921 \\
MonoGS                    & 0.533 & 15.928 & 0.694 \\
Gaussian-SLAM             & 0.399 & 10.523 & 0.928 \\
Ours                      & 0.565 & 17.316 & 0.568 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table}

